Optimized Quantification of Spin Relaxation Times in the Hybrid State

Purpose: The analysis of optimized spin ensemble trajectories for relaxometry in the hybrid state. Methods: First, we constructed visual representations to elucidate the differential equation that governs spin dynamics in hybrid state. Subsequently, numerical optimizations were performed to find spin ensemble trajectories that minimize the Cram\'er-Rao bound for $T_1$-encoding, $T_2$-encoding, and their weighted sum, respectively, followed by a comparison of the Cram\'er-Rao bounds obtained with our optimized spin-trajectories, as well as Look-Locker and multi-spin-echo methods. Finally, we experimentally tested our optimized spin trajectories with in vivo scans of the human brain. Results: After a nonrecurring inversion segment on the southern hemisphere of the Bloch sphere, all optimized spin trajectories pursue repetitive loops on the northern half of the sphere in which the beginning of the first and the end of the last loop deviate from the others. The numerical results obtained in this work align well with intuitive insights gleaned directly from the governing equation. Our results suggest that hybrid-state sequences outperform traditional methods. Moreover, hybrid-state sequences that balance $T_1$- and $T_2$-encoding still result in near optimal signal-to-noise efficiency. Thus, the second parameter can be encoded at virtually no extra cost. Conclusion: We provide insights regarding the optimal encoding processes of spin relaxation times in order to guide the design of robust and efficient pulse sequences. We find that joint acquisitions of $T_1$ and $T_2$ in the hybrid state are substantially more efficient than sequential encoding techniques.

==> Lato-fonts/Makefile <==
## Makefile
## Copyright 2011 Mohamed El Morabity
#
# This work may be distributed and/or modified under the conditions of the LaTeX
# Project Public License, either version 1.3 of this license or (at your option)
# any later version. The latest version of this license is in
# http://www.latex-project.org/lppl.txt and version 1.3 or later is part of all
# distributions of LaTeX version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Mohamed El Morabity
#
# This work consists of all files listed in manifest.txt.

######################
# Fonts informations #
######################

FONT_NAME = lato
FOUNDRY = public
FONT_CODES = fla

# Supported LaTeX encodings
SUPPORTED_ENCODINGS = ot1 t1 ts1
# Supported LaTeX encodings containing small caps
SUPPORTED_SC_ENCODINGS = $(filter-out ts1,$(SUPPORTED_ENCODINGS))
# Custom encodings provided
INPUT_ENCODINGS = $(INPUT_ETX_FILES:$(FONT_NAME)-%.etx=%)


#####################
# Installation root #
#####################

TEXMFHOME = $(shell kpsexpand '$$TEXMFHOME')


###########
# Archive #
###########

ARCHIVE_ROOT = $(FONT_NAME)
ARCHIVE = $(FONT_NAME).zip


###########
# Sources #
###########

TRUETYPE_FILES = $(wildcard *.ttf)

# Fontinst files
FONTINST_FILE = $(FONT_NAME)-drv.tex
FONTINST_MAP_FILE = $(FONT_NAME)-map.tex

# Custom Fontinst encoding files
INPUT_ETX_FILES = $(FONT_NAME)-01.etx $(FONT_NAME)-02.etx $(FONT_NAME)-dotlessj.etx
MTX_FILES = $(FONT_NAME)-fixlatin.mtx $(FONT_NAME)-fixtextcomp.mtx

STYLE_FILES = $(wildcard *.sty)

DOCUMENTATION = $(FONT_NAME).tex $(FONT_NAME).pdf $(FONT_NAME)-samples.tex $(FONT_NAME)-samples.pdf README CHANGES

# Files to be installed in texmf/source
SOURCE_FILES = $(FONTINST_FILE) $(FONTINST_MAP_FILE) $(INPUT_ETX_FILES) $(MTX_FILES) Makefile ttf2type1.pe


###################
# Generated files #
###################

TYPE1_FILES = $(TRUETYPE_FILES:.ttf=.pfb) $(TRUETYPE_FILES:.ttf=-LCDFJ.pfb)
AFM_FILES = $(TYPE1_FILES:.pfb=.afm)

# Fontinst log file
FONTINST_REC_FILE = $(FONT_NAME)-rec.tex

# Metrics files
PL_FILES = $(foreach e,$(INPUT_ENCODINGS),   \
             $(TRUETYPE_FILES:.ttf=-$(e).pl) \
           )
OUTPUT_MTX_FILES = $(PL_FILES:.pl=.mtx)
VPL_FILES = $(foreach e,$(SUPPORTED_ENCODINGS),          \
              $(TRUETYPE_FILES:.ttf=-$(e).vpl)           \
            )                                            \
            $(foreach e,$(SUPPORTED_SC_ENCODINGS),       \
              $(TRUETYPE_FILES:.ttf=-SmallCaps-$(e).vpl) \
            )
TFM_FILES = $(PL_FILES:.pl=.tfm) $(VPL_FILES:.vpl=.tfm)
VF_FILES = $(VPL_FILES:.vpl=.vf)

MAP = $(FONT_NAME).map

# Font definition files
FD_FILES = $(foreach e,$(SUPPORTED_ENCODINGS), \
             $(foreach f,$(FONT_CODES),        \
               $(e)$(f).fd                     \
             )                                 \
           )

# Generated encoding files
ENC_FILES = $(INPUT_ETX_FILES:.etx=.enc)

# Generated files to be installed
GENERATED_FILES = $(TYPE1_FILES) $(AFM_FILES) $(TFM_FILES) $(VF_FILES) $(MAP) $(FD_FILES) $(ENC_FILES)


default: all


all: dist


dist: $(ARCHIVE)


%.pfb %.afm: %.ttf
	fontforge ttf2type1.pe $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%-LCDFJ.pfb: %.pfb
	t1dotlessj $< $@


%-LCDFJ.afm: %-LCDFJ.pfb
	pf2afm $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%.tfm: %.pl
	pltotf $< $@


%.tfm: %.vpl
	vptovf $^ $


%.vf: %.vpl
	vptovf $^ $@


$(FONTINST_REC_FILE): $(AFM_FILES) $(MTX_FILES) $(FONTINST_FILE)
	latex $(FONTINST_FILE)


$(PL_FILES) $(VPL_FILES): $(FONTINST_REC_FILE)


$(MAP): $(FONTINST_REC_FILE) $(FONTINST_MAP_FILE)
	latex $(FONTINST_MAP_FILE)


$(FD_FILES) $(ENC_FILES): $(MAP)


texmf-tree: clean-texmf-tree $(GENERATED_FILES) $(SOURCES_FILES)
	mkdir -p $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{afm,tfm,truetype,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p $(DOCUMENTATION) $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	cp -p $(FD_FILES) $(STYLE_FILES) $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	cp -p $(ENC_FILES) $(ARCHIVE_ROOT)/fonts/enc/dvips/$(FONT_NAME)/
	cp -p $(MAP) $(ARCHIVE_ROOT)/fonts/map/dvips/$(FONT_NAME)/
	cp -p $(AFM_FILES) $(ARCHIVE_ROOT)/fonts/afm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TFM_FILES) $(ARCHIVE_ROOT)/fonts/tfm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TRUETYPE_FILES) $(ARCHIVE_ROOT)/fonts/truetype/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TYPE1_FILES) $(ARCHIVE_ROOT)/fonts/type1/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(VF_FILES) $(ARCHIVE_ROOT)/fonts/vf/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(SOURCE_FILES) $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p README $(ARCHIVE_ROOT)
	cd $(ARCHIVE_ROOT) && find . -type f > manifest.txt


$(ARCHIVE): clean-texmf-tree texmf-tree
	zip -r $@ $(ARCHIVE_ROOT)


install: texmf-tree
	mkdir -p $(TEXMFHOME)
	cp -a $(ARCHIVE_ROOT)/* $(TEXMFHOME)
	texhash
	updmap --enable Map=$(MAP)


uninstall:
	$(RM) -r $(TEXMFHOME)/doc/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/tex/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{afm,tfm,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/source/$(FONT_NAME)/
	updmap --disable $(MAP)
	texhash


clean: clean-texmf-tree
	$(RM) $(TYPE1_FILES) $(AFM_FILES)
	$(RM) $(FONTINST_REC_FILE)
	$(RM) $(PL_FILES) $(TYPE1_FILES:.pfb=.pl)
	$(RM) $(OUTPUT_MTX_FILES) $(TYPE1_FILES:.pfb=.mtx)
	$(RM) $(VPL_FILES)
	$(RM) $(TFM_FILES)
	$(RM) $(VF_FILES)
	$(RM) $(MAP)
	$(RM) $(FD_FILES)
	$(RM) $(ENC_FILES)
	$(RM) $(ARCHIVE)
	$(RM) *~ *.log


clean-texmf-tree:
	$(RM) -r $(ARCHIVE_ROOT)


.PHONY: clean clean-texmf-tree texmf-tree

